A Spectral Algorithm for Inference in Hidden Semi-Markov Models

Hidden semi-Markov models (HSMMs) are latent variable models which allow latent state persistence and can be viewed as a generalization of the popular hidden Markov models (HMMs). In this paper, we introduce a novel spectral algorithm to perform inference in HSMMs. Unlike expectation maximization (EM), our approach correctly estimates the probability of given observation sequence based on a set of training sequences. Our approach is based on estimating moments from the sample, whose number of dimensions depends only logarithmically on the maximum length of the hidden state persistence. Moreover, the algorithm requires only a few matrix inversions and is therefore computationally efficient. Empirical evaluations on synthetic and real data demonstrate the advantage of the algorithm over EM in terms of speed and accuracy, especially for large datasets.

==> RelatedWork.tex <==
The spectral learning algorithms have recently become very popular in machine learning community and have attracted the attention of many researchers %\cite{anima12a, balle11, mossel06}.
These methods provide computationally efficient, local-minimum-free, provably consistent inference and parameter estimation algorithms for latent variable models.

For example, Anandkumar et~al. \cite{anima12b} proposed a spectral method for learning the parameters of a wide class of tree-structured latent graphical models, including Gaussian mixture models, topic models and Latent Dirichlet Allocation. This method is based on a tensor decomposition of certain low order moments, computable directly from data, in order to extract the model parameters. 

However, in many problems the main task is to perform inference and so we would want to avoid explicitly recovering the model parameters and directly compute the quantity of interest. Hsu et~al. \cite{hsu12} proposed an efficient spectral algorithm for HMM for computing marginal and conditional probability distributions of the observed variables.
It is based on the idea of expressing the model in an observable representation, which does not depend on the model parameters and uses easily computable second and third order sample moments to perform inference. However, the proposed algorithm was specific to an HMM topology and it is not straightforward to extend it to other graphical models. 

Parikh et~al. \cite{parikh11} then proposed a spectral algorithm to perform inference in latent tree graphical models with arbitrary topology and later in \cite{parikh12} a general spectral inference framework for latent junction trees. The main idea in both papers was to embed parameters into higher order tensors and then express the model in the observable representation to do the inference.

In this paper, we apply the framework of \cite{parikh12} to perform inference in the HSMM. Note that since our paper addresses a more specific problem than \cite{parikh12}, we shed significantly more light into the details of the spectral algorithm. 

Specifically, our contribution is the derivation of the observable representation for HSMM, where we show a logarithmic size dependency of the sample moments on the longest duration that the state can remain unchanged. We also derive a training scheme, with better computational efficiency and estimation accuracy than was originally presented by \cite{parikh12}. Moreover, through evaluation on synthetic and real datasets we show that the proposed spectral HSMM algorithm is a competitive alternative to the EM approach. 
%Finally, the results of this work were coded into a practical algorithm to be released and used by the machine learning community.

==> secAlgAnalysis.tex <==
In this Section our goal is to analyze the Algorithm \ref{alg1} and study how the rank of matrix $\underset{\bm{\mathsf{X}}_{R_{t+1}}|x_td_t}{\mathbf{T}}$ evolves across iterations. 

\noindent Before we prove Theorem \ref{mainTheoremm}, we will establish certain auxiliary results.

\begin{lemma}
\label{KhatriRao1}
Let $\mathbf{A} \in \mathbb{R}^{m\times n}$ be a matrix with no all-zero columns then $rank\left(\mathbf{I}\odot\mathbf{A}\right) = rank\left(\mathbf{A}\odot\mathbf{I}\right) = n$, where $\odot$ denotes Khatri-Rao product and $\mathbf{I} \in \mathbb{R}^{n\times n}$. 
\end{lemma}

\begin{proof}
Let $\mathbf{K} = \left(\mathbf{I}\odot\mathbf{A}\right) \in \mathbb{R}^{mn\times n}$. By definition of Khatri-Rao product, $\mathbf{K}(:,j) = \mathbf{e}_j\otimes\mathbf{A}(:,j)$, for $j=1,\ldots,n$, which consists of zeros, except for rows $(j-1)m+1,\ldots,(j-1)m+m$, containing the column $\mathbf{A}(:,j)$. Here $\otimes$ denotes Kronecker product and $\mathbf{e}_j$ is everywhere zero except for position $j$ which is $1$. As long as there is no all-zero columns in $\mathbf{A}$, each column of $\mathbf{K}$ is independent of each other and therefore the rank is $n$. Moreover, since the matrix $\mathbf{A}\odot\mathbf{I}$ is a row-permuted version of $\mathbf{A}\odot\mathbf{I}$, their ranks are the same.\qed
\end{proof}

\begin{lemma}
\label{KhatriRao2}
Define a block-row matrix $\mathbf{M} = \left[\mathbf{A}_1 ~\mathbf{A}_2 ~\cdots 
~\mathbf{A}_k\right]\in\mathbb{R}^{m\times kn}$, where each  $\mathbf{A}_i \in \mathbb{R}^{m\times n}$. Define by $r_j, ~j=1,\ldots,n$ the rank of matrix $\left[\mathbf{A}_1(:,j) ~\cdots ~\mathbf{A}_k(:,j)\right]$ composed of $j$th columns of $\mathbf{A}$'s, and let $\mathbf{E} = \left[\mathbf{I} ~\mathbf{I} ~\cdots 
~\mathbf{I}\right]\in\mathbb{R}^{n\times kn}$, where $\mathbf{I} \in \mathbb{R}^{n\times n}$. Then the rank of matrix $\mathbf{W} = \mathbf{M}\odot\mathbf{E} \in \mathbb{R}^{mn\times kn}$, obtained using a Khatri-Rao product, is $\min(mn, \sum_jr_j)$.
\end{lemma}

\begin{proof}
First note that $\mathbf{M}\odot\mathbf{E}$ and $\mathbf{E}\odot\mathbf{M}$ are row permuted version of each other, so they have the same rank. Therefore, consider $\mathbf{W}^{\prime} = \mathbf{E}\odot\mathbf{M} = \left[\mathbf{I}\odot\mathbf{A}_1 \cdots \mathbf{I}\odot\mathbf{A}_k\right]$. Also, note that $\mathbf{e}_j\otimes\left[\mathbf{A}_1(:,j) \cdots ~\mathbf{A}_k(:,j)\right]$, $j=1,\ldots,n$ is a matrix which consists of zeros except for rows $(j-1)m+1,\ldots,(j-1)m+m$ where it contains the columns $\left[\mathbf{A}_1(:,j) ~\cdots ~\mathbf{A}_k(:,j)\right]$. The rank of these columns is $r_j$ and all other columns in $\mathbf{W}$ are independent of them due to the structure of the Khatri-Rao product. Therefore, each set of such columns adds $r_j$ to the total rank. Since the overall rank of $\mathbf{W}$ cannot exceed either the number of rows or columns, we conclude that $rank(\mathbf{W})=\min(mn, \sum_jr_j)$.\qed
\end{proof}


\begin{lemma}
\label{SubsetIndep}
Let $V = \{\mathbf{v}_1,\ldots,\mathbf{v}_n\}$ be a set of independent vectors. Define $\mathbf{u} = \sum_{i=1}^nc_i\mathbf{v}_i$, where coefficients $c_i \neq 0, i=1,\ldots,n$. Define $U$ to be a strict subset of $V$, i.e., $U \subset V $, then a set of vectors $\mathbf{u} \cup U$ is independent.
\end{lemma}

\begin{proof}
Define $\{1,\ldots,n\} = \alpha \cup \bar{\alpha}$, where $\alpha$ denotes a subset of indices for vectors corresponding to $U$. Then we can write $\mathbf{u} = \sum_{i:i\in\alpha}c_i\mathbf{v}_i + \sum_{j:j\in\bar{\alpha}}c_j\mathbf{v}_j$. 

Assuming the opposite, i.e., $\mathbf{u} \cup U$ are dependent, we can write $k_0\mathbf{u} + \sum_{i:i\in\alpha}k_i\mathbf{v}_i = 0$ where $k_0 \neq 0$ and some of $k_i, i\in\alpha$ are also must be non-zero. Substituting the definition of $\mathbf{u}$ and rearranging the terms, we get:
\begin{align*}
k_0\sum_{i:i\in\alpha}(c_i+k_i)\mathbf{v}_i + k_0\sum_{j:j\in\bar{\alpha}}c_j\mathbf{v}_j  = 0.
\end{align*}
\noindent Since $c_j \neq 0, j\in\bar{\alpha}$, the above equation claims the linear dependence of vectors in $V$, which is a contradiction of our assumption and so $\mathbf{u} \cup U$ are independent.\qed
\end{proof}

We now ready to analyze Algorithm \ref{alg1}. It can be verified that \eqref{eq:V} is of the form: 
%
\begin{align}
\label{eq:matrixV}
\mathbf{V} = 
\begin{bmatrix}
\Psi & \vline
\begin{array}{ccc}
\mathbf{I} & &\\
& \ddots &\\
&&\mathbf{I}\\
\hline
\mathbf{0} & \cdots & \mathbf{0}
\end{array}
\end{bmatrix} \in \mathbb{R}^{n_xn_d~\times ~n_xn_d}
\quad\quad\text{where}\quad\Psi = 
\begin{bmatrix}
\text{diag}\left[D(1,:)\right]\mathcal{X}\\
\text{diag}\left[D(2,:)\right]\mathcal{X}\\
\vdots\\
\text{diag}\left[D(n_d,:)\right]\mathcal{X}\\
\end{bmatrix} \in \mathbb{R}^{n_xn_d~\times ~n_x},
\end{align} 
%
\noindent where $\text{diag}\left[D(i,:)\right]$ is the diagonal matrix with $i$th row from $D$ on the diagonal. Note that we can also write $\Psi = \left(D\odot\mathbf{I}\right)\mathcal{X}$. Observe that the rank of $\mathbf{V}$ is $n_xn_d$ because  the $n_x(n_d-1) \times n_x(n_d-1)$ block diagonal matrix delineated in \eqref{eq:matrixV} and the last $n_x\times n_x$ block matrix $\text{diag}\left[D(n_d,:)\right]\mathcal{X}$ in $\Psi$ together comprising $n_xn_d$ independent columns of $\mathbf{V}$. Note that $\text{diag}\left[D(n_d,:)\right]\mathcal{X}$ has rank $n_x$ because $\mathcal{X}$ is full rank and $D(n_d,:)$ is non-zero, which follows from statements 1 and 2 in Assumptions \ref{assumptions}). As a side note observe that the requirement to have $D(n_d,:)$ non-zero implies that there is a non-zero probability of maximum state persistence.  

In analyzing the Algorithm \ref{alg1}, it would be useful to denote the matrices at iteration $i$ in \eqref{eq:expan} and \eqref{eq:prop} as
%
\begin{align*} \underset{x_{t\hspace{-1pt}+\hspace{-1pt}i},~\ldots~,x_{t\hspace{-1pt}+\hspace{-1pt}1}|x_t, d_t}{\mathbf{T}} &= [\mathbf{A}_1^{(i)} ~\cdots ~\mathbf{A}_{n_d}^{(i)}]\\ \underset{x_{t\hspace{-1pt}+\hspace{-1pt}i},~\ldots~,x_{t\hspace{-1pt}+\hspace{-1pt}1},x_t|x_t, d_t}{\mathbf{T}^{\prime}} &= [\mathbf{B}_1^{(i)} ~\cdots~ \mathbf{B}_{n_d}^{(i)}]\\
\underset{x_{t\hspace{-1pt}+\hspace{-1pt}i\hspace{-1pt}+\hspace{-1pt}1},\ldots,x_{t\hspace{-1pt}+\hspace{-1pt}2},x_{t\hspace{-1pt}+\hspace{-1pt}1}|x_t, d_t}{\mathbf{T}} &= [\mathbf{C}_1^{(i)} ~\cdots ~\mathbf{C}_{n_d}^{(i)}].
\end{align*}

\noindent Moreover, utilizing the structure of matrix $\mathbf{V}$ from \eqref{eq:matrixV}, the operations involved in step \eqref{eq:prop} are as follows: 
%
\begin{align}
\label{eq:Vtrans}
\Big[\mathbf{C}_1^{(i)} ~~\mathbf{C}_2^{(i)} ~~\mathbf{C}_3^{(i)} ~~\cdots ~\mathbf{C}_{n_d}^{(i)}\Big] = \Big[[\mathbf{B}_1^{(i)} ~\cdots~ \mathbf{B}_{n_d}^{(i)}]\Psi ~~~\mathbf{B}_1^{(i)} ~~\mathbf{B}_2^{(i)} ~~\cdots ~~\mathbf{B}_{n_d-1}^{(i)}\Big].
\end{align}


\noindent With the above information we can now present the proof of Theorem \ref{mainTheoremm}:

\begin{proof}
At the start of the algorithm, we have $\underset{x_{t+1}|x_t, d_t}{\mathbf{T}} = \left[\mathcal{X}~\mathbf{I}~\cdots~\mathbf{I}\right] = [\mathbf{A}_1^{(1)} \cdots \mathbf{A}_{n_d}^{(1)}]$, which has rank $n_x$. The rank of matrix $\left[\mathbf{A}_1^{(1)}(:,l)\cdots \mathbf{A}_{n_d}^{(1)}(:,l)\right]$ for $l=1,\ldots, n_x$ is $r_l = 2$ since among all the columns only two of them are independent. Therefore, according to Lemma \ref{KhatriRao2}, the result of operations in \eqref{eq:expan}, has rank $\sum_{l}r_l = 2n_x$. Moreover, we note that since $[\mathbf{B}_1^{(1)} ~\mathbf{B}_2^{(1)} ~\cdots ~\mathbf{B}_{n_d}^{(1)}] = [\mathcal{X}\hspace{-1pt}\odot\hspace{-1pt}\mathbf{I} ~~\mathbf{I}\hspace{-1pt}\odot\hspace{-1pt}\mathbf{I}~ \cdots~ \mathbf{I}\hspace{-1pt}\odot\hspace{-1pt}\mathbf{I}]$, it can be seen that its $2n_x$ independent vectors can be formed by the columns $[\mathbf{B}_1^{(1)} ~\mathbf{B}_2^{(1)}]$, so that the rank of $\left[\mathbf{B}_1^{(1)}(:,l) \cdots \mathbf{B}_{n_d}^{(1)}(:,l)\right]$ for $l=1,\ldots, n_x$ is $2$.

Next, since the rank of $\mathbf{V}$ is $n_xn_d$, the operations in \eqref{eq:prop} produce matrix $[\mathbf{C}_1^{(1)}  ~\mathbf{C}_2^{(1)} ~\cdots ~\mathbf{C}_{n_d}^{(1)}]$ with the rank still being $2n_x$. Moreover, the columns of $\mathbf{C}_1^{(1)}$ are linearly dependent on the rest of the columns, $[\mathbf{C}_2^{(1)} ~\cdots ~\mathbf{C}_{n_d}^{(1)}]$, due to \eqref{eq:Vtrans}. However, the rank of $\left[\mathbf{C}_1^{(1)}(:,l) \cdots \mathbf{C}_{n_d}^{(1)}(:,l)\right]$ is now $r_l = 3$ for $l=1,\ldots, n_x$ . To understand this, note that 
%
\begin{align*}
[\mathbf{B}_1^{(1)} ~~\mathbf{B}_2^{(1)}~\cdots ~ \mathbf{B}_{n_d}^{1}] &= [\mathcal{X}\hspace{-2pt}\odot\hspace{-2pt}\mathbf{I} ~~\mathbf{I}\hspace{-2pt}\odot\hspace{-2pt}\mathbf{I}~ \cdots~ \mathbf{I}\hspace{-2pt}\odot\hspace{-2pt}\mathbf{I}]\\
[\mathbf{C}_1^{(1)}~~\mathbf{C}_2^{(1)}~~\mathbf{C}_3^{(1)}~\cdots~ \mathbf{C}_{n_d}^{(1)}] &= [\mathbf{C}_1^{(1)}~ ~\mathcal{X}\hspace{-2pt}\odot\hspace{-2pt}\mathbf{I} ~~\mathbf{I}\hspace{-2pt}\odot\hspace{-2pt}\mathbf{I}~ \cdots~ \mathbf{I}\hspace{-2pt}\odot\hspace{-2pt}\mathbf{I}],
\end{align*}
\noindent where, according to \eqref{eq:Vtrans}, $\mathbf{C}_1^{(1)} = [\mathbf{B}_1^{(1)} \cdots \mathbf{B}_{n_d}^{(1)}]\Psi$. As we established before, the rank of $\left[\mathbf{C}_2^{(1)}(:,l) \cdots \mathbf{C}_{n_d}^{(1)}(:,l)\right] = \left[\mathbf{B}_1^{(1)}(:,l) \cdots \mathbf{B}_{n_{d-1}}^{(1)}(:,l)\right]$ is $r_l=2$. Moreover, it can also be checked that $\mathbf{C}_1^{(1)}(:,l)$ is independent of $\left[\mathbf{C}_2^{(1)}(:,l) \cdots \mathbf{C}_{n_d}^{(1)}(:,l)\right]$ due to Lemma \ref{SubsetIndep}. Clearly, then the cumulative rank of $\left[\mathbf{C}_1^{(1)}(:,l) \cdots \mathbf{C}_{n_d}^{(1)}(:,l)\right]$ is $3$ for $l=1,\ldots, n_x$.

To generalize, if at the iteration $i$ the rank of $\left[\mathbf{A}_1^{(i)} \cdots \mathbf{A}_{n_d}^{(i)}\right]$ is $in_x$ while the rank of $\left[\mathbf{A}_1^{(i)}(:,l) \cdots \mathbf{A}_{n_d}^{(i)}(:,l)\right]$ is $(i+1)$, then the operations in step \eqref{eq:expan} produce $\left[\mathbf{B}_1^{(i)} \cdots \mathbf{B}_{n_d}^{(i)}\right]$ having rank $(i+1)n_x$ due to Lemma \ref{KhatriRao2}. The step in \eqref{eq:prop} keeps the rank of $\left[\mathbf{C}_1^{(i)} \cdots \mathbf{C}_{n_d}^{(i)}\right]$ at $(i+1)n_x$ due to the full rank structure of $\mathbf{V}$. At the same time, this step increases the rank of $\left[\mathbf{C}_1^{(i)}(:,l) \cdots \mathbf{C}_{n_d}^{(i)}(:,l)\right]$ to $(i+2)$ due to Lemma \ref{SubsetIndep}, i.e., independence of $\mathbf{C}_1^{(i)}(:,l)$ from $\left[\mathbf{C}_2^{(i)}(:,l) \cdots \mathbf{C}_{n_d}^{(i)}(:,l)\right]$ with the latter having the rank $(i+1)$. Therefore, each iteration increases the rank of matrix $\mathbf{T}$ by $n_x$ and so after $2 \leq \ell  \leq n_d$ steps the rank of the resulting matrix $\underset{\bm{\mathsf{X}}_{R_{t+1}}|x_td_t}{\mathbf{T}}$ is $\ell n_x$. 

Note that if $\ell =1$ then the Algorithm \ref{alg1} is not executed and returns the trivial $\underset{x_{t+1}|x_t, d_t}{\mathbf{T}}$ with rank $n_x$. On the other hand, if $\ell  > n_d$ then the rank of $\underset{\bm{\mathsf{X}}_{R_{t+1}}|x_td_t}{\mathbf{T}}$ is $n_xn_d$ since this is the number of columns in that matrix and so is the maximum achievable rank.\qed
\end{proof}




